RCOT: Detecting and Rectifying Factual Inconsistency in Reasoning by Reversing Chain-of-Thought

Large language Models (LLMs) have achieved promising performance on arithmetic reasoning tasks by incorporating step-by-step chain-of-thought (CoT) prompting. However, LLMs face challenges in maintaining factual consistency during reasoning, exhibiting tendencies to condition overlooking, question misinterpretation, and condition hallucination over given problems. Existing methods use coarse-grained feedback (e.g., whether the answer is correct) to improve factual consistency. In this work, we propose RCoT (Reversing Chain-of-Thought), a novel method to improve LLMs' reasoning abilities by automatically detecting and rectifying factual inconsistency in LLMs, generated solutions. To detect factual inconsistency, RCoT first asks LLMs to reconstruct the problem based on generated solutions. Then fine-grained comparisons between the original problem and the reconstructed problem expose the factual inconsistency in the original solutions. To rectify the solution, RCoT formulates detected factual inconsistency into fine-grained feedback to guide LLMs in revising solutions. Experimental results demonstrate improvements of RCoT over standard CoT, Self-Consistency and Self-Refine across seven arithmetic datasets. Moreover, we find that manually written fine-grained feedback can dramatically improve LLMs' reasoning abilities (e.g., ChatGPT reaches 94.6% accuracy on GSM8K), encouraging the community to further explore the fine-grained feedback generation methods.

==> overlook_example.tex <==
\begin{center}
\begin{tcolorbox}[title={\textcolor{cyan}{Original Problem:} \textcolor{red}{The deadline is Jun 1, 2021, which is 2 days away from now.} What is the date a month ago in MM/DD/YYYY? Answer Choices: (A) 04/30/2021 (B) 02/19/2021 (C) 05/01/2021 (D) 05/09/2021 (E) 07/06/2021 (F) 08/03/2021 \textcolor{yellow}{Date}\\
\textcolor{cyan}{Reconstrated Problem:} What is the date that is one month before the deadline of June 1, 2021, written in the format MM/DD/YYYY? Answer Choices: (A) 04/30/2021 (B) 02/19/2021 (C) 05/01/2021 (D) 05/09/2021 (E) 07/06/2021 (F) 08/03/2021}]
\normalsize\textbf{Original Solution:}\\
\small{First, we need to find the date that is one month before the deadline of June 1, 2021. To do this, we can subtract one month from the deadline date. \\
\textcolor{red}{June 1, 2021 - 1 month = May 1, 2021 \\
So, the date that is one month before the deadline is May 1, 2021.} \\
Next, we need to write this date in the format MM/DD/YYYY. \\
May 1, 2021 = 05/01/2021 \\
Therefore, the answer is (C) 05/01/2021.\textcolor{red}{\ding{55}}}
\end{tcolorbox}
\captionof{figure}{An example showing that LLMs \vtwo{} condition.}
\label{overlooked_example}
\end{center}

==> prompt_temp.tex <==
\begin{tcolorbox}[colback=blue!-15!white,colframe=blue!65!yellow,fonttitle=\bfseries,title=\hspace{5.6cm}\textbf{Prompt}]
\normalsize\textbf{Problem Reconstruction}\\
\small{Give the concrete prompt (problem) that can generate this answer. The problem should contain all basic and necessary information and correspond to the answer. The problem can only ask for one result.}\\
\\
\normalsize\textbf{Problem Decomposition}\\
\small{Please list the conditions of the problem. There may be multiple conditions.\\
Do not list conditions not related to calculations, but list all necessary conditions.\\
The format should be:\\
Conditions:\\
This is your output of conditions. Each line is one condition.}\\\\
\normalsize\textbf{Condition Comparison}\\
\small{Given a candidate condition: "\{condition\}"\\
\\
Here is a condition list:"\{condition list\}"\\
\\
From a mathematical point of view, can this candidate condition be deduced from the condition list?\\
Please illustrate your reason and answer "yes" or "no".}\\\\
\normalsize\textbf{Question Comparison}\\
\small{Q1: "\{original problem\}"\\
Q2: "\{reconstructed problem\}"\\

From a mathematical point of view, are these two problems ask the same thing at the end?\\
Please illustrate your reason and answer "yes" or "no".}\\\\
\normalsize\textbf{Fine-grained Feedback and Revision}\\
\small{Here are the mistakes and reasons in your answer to the problem.\\\\
\textbf{Overlooked Conditions:}\\
You have ignored some real conditions:\\
"\{condition\}"\\
The real problem has the conditions:\\
"\{condition list\}"\\
You should consider all real conditions in the problem.\\
Here are detailed reasons:\\
"\{illustration\}"}\\\\
\small{\textbf{Hallucinated Conditions}\\
You use some wrong candidate conditions:\\
"\{condition\}"\\
They all can not be deduced from the true condition list.\\
The real problem has the conditions:\\
"\{condition list\}"\\
You should consider all real conditions in the problem.\\
Here are detailed reasons:\\
"\{illustration\}"}\\\\
\small{\textbf{Misinterpreted Question}\\
You misunderstood the question.\\
You think the question is "\{reconstructed question\}".\\
But the real question is "\{original question\}".\\
They are different. You should consider the real question.}
\end{tcolorbox}
\captionof{figure}{All prompts in our method}
\label{promptfigure}

==> quan_table.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\label{table20}
\vspace{-5mm}
\renewcommand{\arraystretch}{1.3}
{
\captionof{table}{\textbf{Found:} RCoT could find the reasons for errors. \textbf{Not Found:} RCoT cannot find the errors. \textbf{Other errors:} such as computation error, logical error and so on.}
\begin{tabular}{lccc}
\toprule
Type              & Found & Not Found & total \\ \midrule
Overlooking       & 5          & 1                & 6     \\ \midrule
Hallucinating     & 16         & 15               & 31    \\ \midrule
Misinterpreting & 5          & 3                & 8     \\ \midrule
Other errors      & 0          & 55               & 55    \\ \bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{wraptable}
